Efficient Reinforcement Learning in Factored MDPs with Application to Constrained RL

Reinforcement learning (RL) in episodic, factored Markov decision processes (FMDPs) is studied. We propose an algorithm called FMDP-BF, which leverages the factorization structure of FMDP. The regret of FMDP-BF is shown to be exponentially smaller than that of optimal algorithms designed for non-factored MDPs, and improves on the best previous result for FMDPs~\citep{osband2014near} by a factored of $\sqrt{H|\mathcal{S}_i|}$, where $|\mathcal{S}_i|$ is the cardinality of the factored state subspace and $H$ is the planning horizon. To show the optimality of our bounds, we also provide a lower bound for FMDP, which indicates that our algorithm is near-optimal w.r.t. timestep $T$, horizon $H$ and factored state-action subspace cardinality. Finally, as an application, we study a new formulation of constrained RL, known as RL with knapsack constraints (RLwK), and provides the first sample-efficient algorithm based on FMDP-BF.

==> UCB_Hoeffding.tex <==
\section{Algorithm with Hoeffding-type Bonus}
\label{sec: algorithm with Hoeffding-type bonus}
In this section, we introduce our algorithm with Hoeffding-type confidence bonus and present the corresponding regret bound. Our algorithm, which is described in Algorithm~\ref{alg:Algorithm with Hoeffding-type Bonus}, is related to UCBVI-CH algorithm~\cite{azar2017minimax}, in the sense that Algorithm~\ref{alg:Algorithm with Hoeffding-type Bonus} reduces to UCBVI-CH if we consider a flat MDP with $m=n=d=1$. Our contribution is 
a more refined design of confidence bonus for factored MDP and the analysis which lead to a tight regret bound independent of the cardinality of the whole state space $|\mathcal{S}|$.

\subsection{Algorithm}
 \begin{algorithm}[tbh]
\caption{FMDP-CH}
\label{alg:Algorithm with Hoeffding-type Bonus}
  \begin{algorithmic}[5]
    \State  \textbf{Input}: $\delta$, 
    \State history data $\mathcal{L} = \emptyset$, initialize $N((s,a)[Z_i]) = 0$ for any factored set $Z_i$ and $(s,a)[Z_i] \in \mathcal{X}[Z_i]$
    %\State Run Alg. \ref{alg:warm-up} for warm-up and update the counter.
	\For {episode $k=1,2,...$}
        \State Set $\hat{V}_{k,H+1}(s) = 0$ for all $s$.
        \State Estimate $\hat{R}_{k,i}(s,a)$ with empirical mean value if $N_{k-1}((s,a)[Z^R_i]) >0$, otherwise $\hat{R}_{k,i}(s,a) = 1$, then calculate $\hat{R}(s,a) = \frac{1}{m}\sum_{i=1}^{m}\hat{R}_i((s,a)[Z^R_i])$
        \State Let $\mathcal{K}_P = \left\{(s, a) \in \mathcal{S} \times \mathcal{A}, \cup_{i\in [n]} N_{k}((s, a)[Z^P_i])>0\right\}$
        \State Estimate $\hat{P}_k(\cdot|s,a)$ with empirical mean value for all $(s,a) \in \mathcal{K}_P$
    	\For {horizon $h=H,H-1,...,1$}
    	    \For {all $(s,a) \in \mathcal{S} \times \mathcal{A}$ }
                \If {$(s.a) \in \mathcal{K}_P$}
                    \State $\hat{Q}_{k,h}(s,a) = \min\{H, \hat{R}_{k}(s,a) + CB_k(s,a)+ \hat{\mathbb{P}}_{k} \hat{V}_{k,h+1}(s,a)\}$
                \Else
                    \State $\hat{Q}_{k,h}(s,a) = H$
                \EndIf
                \State $\hat{V}_{k, h}(s)=\max _{a \in \mathcal{A}} \hat{Q}_{k, h}(s, a)$
    		\EndFor
    	\EndFor
        \For{step $h = 1,\cdots,H$}
		    \State Take action $a_{k,h} = \arg \max_a \hat{Q}_{k,h}(s_{k,h},a)$
		\EndFor
		\State Update history trajectory $\mathcal{L} = \mathcal{L} \bigcup \{s_{k,h},a_{k,h},r_{k,h},s_{k,h+1}\}_{h=1,2,...,H}$, and update history counter $N_{k-1}((s,a)[Z_i])$.
	\EndFor
  \end{algorithmic}
\end{algorithm}
Our algorithm follows the principle of "optimism in the face of uncertainty", which is a standard principle and has been applied to many previous algorithms~\cite{dann2017unifying,azar2017minimax,jin2018q,dong2019q,zanette2019tighter}. Let $N_{k}((s,a)[Z])$ denote the number of steps that the agent encounters $(s,a)[Z]$ during the first $k$ episodes, and $N_{k}((s,a)[Z_j],s_j)$ denotes the number of steps that the agent transits to a state with $s[j] = s_j$ after encountering $(s,a)[Z_j]$ during the first $k$ episodes. In episode $k$, we estimate the mean value of each factored reward $R_i$ and each factored transition $\mathbb{P}_{i}$ with empirical mean value $\hat{R}_{k,i}$ and $\hat{\mathbb{P}}_{k,i}$ respectively. To be more specific, $\hat{R}_{k,i}((s,a)[Z^R_i]) = \frac{\sum_{t \leq (k-1)H}\mathbbm{1}\left[(s,a)_{t}[Z^R_i] = (s,a)[Z^R_i]\right] \cdot r_{t,i}(s_{t},a_{t})}{N_{k-1}((s,a)[Z^R_i])}$, where $r_{t,i}$ denotes the reward $R_i$ sampled in step $t$, and   $\hat{\mathbb{P}}_{k,j}\left(s[j]|(s,a)[Z^P_j]\right) = \frac{N_{k-1}((s,a)[Z^P_j],s[j])}{N_{k-1}((s,a)[Z^P_j])}$. After that, we construct the optimistic MDP $\hat{M}$ based on the estimated rewards and transition functions. For a certain $(s,a)$ pair, the transition function and reward function are defined as $\hat{R}_k(s,a) = \frac{1}{m}\sum_{i=1}^{m}\hat{R}_{k,i}((s,a)[Z^R_i])$ and $\hat{\mathbb{P}}_k(s' \mid s,a)=\prod_{j=1}^{n} \hat{\mathbb{P}}_{k,j}\left(s'[j] \mid (s,a)\left[Z^P_{j}\right]\right)$.

To guarantee optimism, we need to add confidence bonus to the estimated value function $\hat{V}$, so that $\hat{V}_{k,h}(s) \geq V^*_h(s)$ holds for any $k \in [K]$, $h \in [H]$ and $s \in \mathcal{S}$. Following the previous framework, the confidence bonus need to tightly characterize the estimation error of the one-step backup $\bar{R}(s,a) +\mathbb{P}V^*_h(s,a)$, or in other words, to compensate the estimation error $\left(\hat{R} - \bar{R}\right)(s,a)$ and $\left(\hat{\mathbb{P}}- \mathbb{P}\right)V^*_h(s,a)$ respectively.  

For the estimation error of rewards $\hat{R}_k(s_{k,h},a_{k,h}) - \bar{R}(s_{k,h},a_{k,h})$, since the reward is defined as the average of $m$ factored rewards, it is not hard to decompose the estimation error of $\bar{R}(s,a)$ to the average of the estimation error of each factored rewards. We define $L^R_i = \log \left( 18 m T \left|\mathcal{X}[Z_i^R]\right|/\delta \right)$. In that case, we separately construct the confidence bonus of each factored reward $R_i$ in the following way:
  \begin{align}
  \label{eqn: confidence bonus for each factored reward}
    CB^R_{k,Z_i^R}(s,a) =  &\sqrt{\frac{2 L^R_i}{N_{k-1}((s,a)[Z^R_i])}},\quad i \in [m] 
  \end{align}
  
For the estimation error of transition $\left(\hat{\mathbb{P}}_{k} - \mathbb{P}\right)V^*_{h+1}(s_{k,h},a_{k,h})$, the main difficulty to compensate  this error is that $\hat{\mathbb{P}}_k$ is the multiplication of $n$ estimated transition dynamics $\hat{\mathbb{P}}_{k,i}$. In that case, the estimation error $\left(\hat{\mathbb{P}}_{k} - \mathbb{P}\right)V^*_{h+1}(s_{k,h},a_{k,h})$ may be calculated as the multiplication of $n$ estimation error for each factored transition $\hat{\mathbb{P}}_{k,i}$. Luckily, we find the following lemma useful to tackle this issue.

\begin{lemma}
    \label{lemma: decomposition of value estimation error}
   Let the transition function class $\mathbb{P} \in \mathbb{P}_{\mathcal{X},\mathcal{S}}$ be factored over $\mathcal{X} = \mathcal{X}_1 \times \cdots \times \mathcal{X}_n$, and $\mathcal{S} = \mathcal{S}_1 \times \cdots \times \mathcal{S}_n$ with scope $Z^P_1,\cdots,Z^P_n$. For a given function $V: \mathcal{S}\rightarrow \mathbb{R}$, the estimation error of one-step value $|(\hat{\mathbb{P}}_k - \mathbb{P})V(s,a)|$ can be decomposed in the following way:
   \begin{align*}
       |(\hat{\mathbb{P}}_k - \mathbb{P})V(s,a)| 
        \leq& \sum_{i=1}^{n} \left|  (\hat{\mathbb{P}}_{k,i} - \mathbb{P}_{i}) \left(\prod_{j\neq i, j=1}^{n} \mathbb{P}_{j}\right)V(s,a)\right| \notag\\
        &+ \sum_{i=1}^{n}\sum_{j\neq i,j=1}^{n} |V|_{\infty}\left|\left(\hat{\mathbb{P}}_{k,i} - \mathbb{P}_i\right)(\cdot|(s,a)[Z^P_i])\right|_1 \cdot \left|\left(\hat{\mathbb{P}}_{k,j} - \mathbb{P}_j\right)(\cdot|(s,a)[Z^P_j])\right|_1
   \end{align*}
\end{lemma}

The second part in the RHS can be shown to be a lower order terms that doesn't influence the main factors in the regret. (TODO: higher order terms?) With the help of Lemma~\ref{lemma: decomposition of value estimation error}, we successfully decompose the estimation error $\left(\hat{\mathbb{P}}_{k} - \mathbb{P}\right)V^*_{h+1}(s_{k,h},a_{k,h})$ into an additive form, thus we can construct the confidence bonus for each factored transition $\mathbb{P}_i$ in the similar manner of that for rewards. We define $\phi_{k,i}(s,a)=\sqrt{\frac{4|\mathcal{S}_i|L^P}{N_{k-1}((s,a)[Z^P_i])}} + \frac{4|\mathcal{S}_i|L}{3N_{k-1}(s,a)}$ and $L^P = \log \left( 18 n T SA/\delta \right)$ for short. Following the idea of Lemma~\ref{lemma: decomposition of value estimation error}, we separately construct the confidence bonus of scope $Z^P_i$ for transition estimation:
  \begin{align}
    \label{eqn: confidence bonus for each factored transition}
    CB^P_{k,Z_i^P}(s,a) = & \sqrt{\frac{2H^2 L^P}{N_{k-1}((s,a)[Z^P_i])}} + H \phi_{k,i}(s,a)\sum_{j=1,j\neq i}^{n} \phi_{k,j}(s,a), \quad i \in [n]
  \end{align}
 We define the confidence bonus as the summation of all confidence bonus for rewards and transition, i.e. $CB_{k}(s,a) = \frac{1}{m}\sum_{i=1}^{m} CB^R_{k,Z^R_i}(s,a) + \sum_{j=1}^{n} CB^P_{k,Z^P_j}(s,a)$.
 
\subsection{Regret}
We propose the following regret upper bound for Alg.~\ref{alg:Algorithm with Hoeffding-type Bonus}.
\begin{theorem}
\label{thm: Hoeffding regret}
With prob. $1-\delta$, the regret of Alg.~\ref{alg:Algorithm with Hoeffding-type Bonus} is upper bounded by $$Reg(T) = \mathcal{O} \left(\frac{1}{m}\sum_{i=1}^{m} \sqrt{\left|\mathcal{X}[Z_i^R]\right|T \log (mT|\mathcal{X}[Z^R_i]|/\delta) } + \sum_{j=1}^{n} H \sqrt{\left|\mathcal{X}[Z_j^P]\right|T \log (nTSA/\delta) }\right)$$
Here $\mathcal{O}$ hides the lower order terms with respect to $T$.
\end{theorem}

(TODO: more clean version)

Note that the regret bound doesn't depend on the cardinalities of state and action space, but only has square root dependence on the cardinality of each factored subspace $X[Z_i]$. By leveraging the structure of factored MDP, it is possible to achieve regret that scales exponentially smaller compared with that of UCBVI~\cite{azar2017minimax}. Previously the best regret bound for episodic factored MDP is achieved by \cite{osband2014near}. When transformed to our setting, it is:$$\mathcal{O} \left(\frac{1}{m}\sum_{i=1}^{m} \sqrt{|\mathcal{X}[Z_i^R]|T \log (mT|\mathcal{X}[Z_i^R]|/\delta) } + \sum_{j=1}^{n} H \sqrt{|\mathcal{X}[Z_j^P]||\mathcal{S}_j|T \log (nT|\mathcal{X}[Z_j^P]|/\delta) }\right).$$ Compared with their bound, we also improved by a factor of $\sqrt{|\mathcal{S}_j|}$.

\iffalse
\subsection{Proof Sketch}
We defer the detailed proof to Section~\ref{section: proof of Hoeffding bound} and only sketch the proof in this subsection. Following the standard regret decomposition technique~\cite{dann2017unifying,azar2017minimax,zanette2019tighter}, we can decompose the regret in the following way:
\begin{align}
        &Reg(T) \\
        \label{eqn: estimation error in Hoeffding regret decomposition}
        \leq &\sum_{k\in [K],h \in [H]} \Bigg (\left(\hat{R}_k(s_{k,h},a_{k,h}) - \bar{R}(s_{k,h},a_{k,h})\right)
        + \left(\hat{\mathbb{P}}_{k} - \mathbb{P}\right)V^*_{h+1}(s_{k,h},a_{k,h})\\ 
       &+ \left(\mathbb{P} \left(\hat{V}_{k,h+1} -  V^{\pi_k}_{h+1}\right)(s_{k,h},a_{k,h}) - \left(\hat{V}_{k,h+1} -  V^{\pi_k}_{h+1}\right)(s_{k,h+1})\right) \\
       &+ \left(\hat{\mathbb{P}}_{k} - \mathbb{P}\right)\left(\hat{V}_{k,h+1}-V^*_{h+1}\right)\left(s_{k,h},a_{k,h}\right) \\
       &+ CB_k(s_{k,h},\pi^*_h(s ))\Bigg),
   \end{align}
   where $\mathbb{P}V(s,a)$ is a shorthand of $\sum_{s'} \mathbb{P}(s'|s,a)V(s')$ for each given $\mathbb{P}$ and $V$. 
   
   We only sketch the proof of estimation error terms (Eqn.~\ref{eqn: estimation error in Hoeffding regret decomposition}), which both contribute to the main factor in the regret bound and influence the construction of confidence bonus for optimism. The first term $\hat{R}_k(s_{k,h},a_{k,h}) - \bar{R}(s_{k,h},a_{k,h})$ is the estimation error of reward. Since the reward is defined as the average of $m$ factored rewards. It is not hard to decompose the estimation error of $\bar{R}(s,a)$ to the average of the estimation error of each factored rewards. With the help of standard concentration theorem such as Hoeffding's inequality, we can upper bound the regret caused by the estimation error of rewards, which finally results to the first part of the regret in Thm.~\ref{thm: Hoeffding regret}. 
   
   %$\mathbb{P} \left(\hat{V}_{k,h+1} -  V^{\pi_k}_{h+1}\right)(s_{k,h},a_{k,h}) - \left(\hat{V}_{k,h+1} -  V^{\pi_k}_{h+1}\right)(s_{k,h+1})$ can be regarded as a sequence of martingale differences, the summation of which can be bounded by Azuma's inequality. $\left(\hat{\mathbb{P}}_{k} - \mathbb{P}\right)\left(\hat{V}_{k,h+1}-V^*_{h+1}\right)\left(s_{k,h},a_{k,h}\right)$ is a lower order term, and we defer the detailed technical proof to Section~\ref{section: proof of Hoeffding bound}. 
   
   $\left(\hat{\mathbb{P}}_{k} - \mathbb{P}\right)V^*_{h+1}(s_{k,h},a_{k,h})$ is the estimation error of transition dynamics. The main difficulty tp bound the regret due to this term is that $\hat{\mathbb{P}}_k$ is the multiplication of $n$ estimated transition dynamics $\hat{\mathbb{P}}_{k,i}$. In that case, the estimation error $\left(\hat{\mathbb{P}}_{k} - \mathbb{P}\right)V^*_{h+1}(s_{k,h},a_{k,h})$ may be calculated as the multiplication of $n$ estimation error for each factored transition $\hat{\mathbb{P}}_{k,i}$. Luckily, we find the following lemma useful to tackle this issue.
   
\begin{lemma}
    \label{lemma: decomposition of value estimation error}
   Let the transition function class $\mathbb{P} \in \mathbb{P}_{\mathcal{X},\mathcal{S}}$ be factored over $\mathcal{X} = \mathcal{X}_1 \times \cdots \times \mathcal{X}_n$, and $\mathcal{S} = \mathcal{S}_1 \times \cdots \times \mathcal{S}_n$ with scope $Z^P_1,\cdots,Z^P_m$. For a given value function $V(s)$, the estimation error of one-step value $|(\hat{\mathbb{P}}_k - \mathbb{P})V(s,a)|$ can be decomposed in the following way:
   \begin{align*}
       |(\hat{\mathbb{P}}_k - \mathbb{P})V(s,a)| 
        \leq& \sum_{i=1}^{n} \left|  (\hat{\mathbb{P}}_{k,i} - \mathbb{P}_{i}) \left(\prod_{j\neq i, j=1}^{n} \mathbb{P}_{j}\right)V(s,a)\right| \notag\\
        &+ \sum_{i=1}^{n}\sum_{j\neq i,j=1}^{n} |V|_{\infty}\left|\left(\hat{\mathbb{P}}_{k,i} - \mathbb{P}_i\right)(\cdot|(s,a)[Z^P_i])\right|_1 \cdot \left|\left(\hat{\mathbb{P}}_{k,j} - \mathbb{P}_j\right)(\cdot|(s,a)[Z^P_j])\right|_1
   \end{align*}
\end{lemma}

Please see Section~\ref{section: decomposition lemma} for the detailed proof. The first term in Lemma~\ref{lemma: decomposition of value estimation error} can be regarded as the estimation error of each factored transition $\hat{\mathbb{P}}_{k,i}$. For the second part, we can show that the summation is a lower-order term w.r.t $T$. With the help of Lemma~\ref{lemma: decomposition of value estimation error}, we successfully decompose $\left(\hat{\mathbb{P}}_{k} - \mathbb{P}\right)V^*_{h+1}(s_{k,h},a_{k,h})$ as the summation of the estimation error of each factored transition dynamics. Besides, this lemma is also the reason why the confidence bonus is designed as the formula of Eqn.~\ref{eqn: confidence bonus for each factored transition}.
 \fi
